Mining Network Events using Traceroute Empathy

In the never-ending quest for tools that enable an ISP to smooth troubleshooting and improve awareness of network behavior, very much effort has been devoted in the collection of data by active and passive measurement at the data plane and at the control plane level. Exploitation of collected data has been mostly focused on anomaly detection and on root-cause analysis. Our objective is somewhat in the middle. We consider traceroutes collected by a network of probes and aim at introducing a practically applicable methodology to quickly spot measurements that are related to high-impact events happened in the network. Such filtering process eases further in- depth human-based analysis, for example with visual tools which are effective only when handling a limited amount of data. We introduce the empathy relation between traceroutes as the cornerstone of our formal characterization of the traceroutes related to a network event. Based on this model, we describe an algorithm that finds traceroutes related to high-impact events in an arbitrary set of measurements. Evidence of the effectiveness of our approach is given by experimental results produced on real-world data.

==> 035-net_events.tex <==
\section{Modeling Traceroute Path Changes}\label{sec:changes}

\begin{figure}
   \centering
   \includegraphics[scale=.85]{path-example}
   \caption{An example of two traceroute paths from $s$ to $d$ collected at 
different time instants $t$ and $t+1$. Gray 
   lines represent edges of graph $G$.}
   \label{fig:path-example}
\end{figure}

We now introduce a few formal tools to examine how 
traceroute paths change as a consequence of network events. We use these tools 
to formulate assumptions on path changes, which in turn we 
exploit in searching for network events.

\subsection{Common and Changed Portions of Traceroutes}\label{sec:delta}
Let $i=(s,d)$, with $s\in V$ and $d\in V$, and consider traceroute paths
$p_i(t)=\left<v_1\ v_2\ \dots\ v_n\right>$ and
$p_i(t+1)=\left<v'_1\ v'_2\ \dots\ v'_m\right>$, resulting from 
executing \texttt{traceroute}s from $s$ to $d$ at the consecutive time instants 
$t$ and $t+1$.
Assume that $v_1=v'_1=s$ and $p_i(t)\neq 
p_i(t+1)$. An example of two such paths is shown in 
Fig.~\ref{fig:path-example}, where
$i=(1,9)$, $p_i(t)=\left<1\ 2\ 3\ 4\ 5\ 8\ 9\right>$, and
$p_i(t+1)=\left<1\ 2\ 6\ 7\ 8\ 9\right>$.
%
Paths $p_i(t)$ and $p_i(t+1)$ may have one or more vertices in 
common.
Let $c^\mathrm{head}$ denote the \emph{common prefix} of 
$p_i(t)$ and 
$p_i(t+1)$, namely the maximal subsequence
$\left<v_1\ v_2\ \dots\ v_j\right>$ 
of 
$p_i(t)$ and $p_i(t+1)$ such that $j\leq\min(n,m)$ and $v_k=v'_k$ for $k=1, 
\dots, j$ (note that this is obvious for $k=1$, since $v_1=v'_1=s$). For 
example, for the paths in 
Fig.~\ref{fig:path-example} we have that
$c^{\mathrm{head}}=\left<1\ 2\right>$.
A few properties apply to the common prefix. 
First 
of all, it is always $c^{\mathrm{head}}\neq \left<\right>$, because at 
least 
vertex $v_1=s$ will always be in $c^{\mathrm{head}}$.
In addition, since $p_i(t)\neq p_i(t+1)$, it will always be 
$c^\mathrm{head}\neq p_i(t)$ or
$c^\mathrm{head}\neq p_i(t+1)$. However, when at 
least one of $p_i(t)$ and $p_i(t+1)$ does not end at the intended 
destination $d$, the common prefix may coincide with one of the paths, namely it 
can 
be either $c^\mathrm{head}=p_i(t)$ or 
$c^\mathrm{head}=p_i(t+1)$.

Similarly, let $c^\mathrm{tail}$ denote the \emph{common suffix} of 
$p_i(t)$ 
and $p_i(t+1)$, namely the maximal subsequence
$\left<v_h\ v_{h+1}\ \dots\ v_n\right>$ 
of $p_i(t)$ of length $n-h+1$ and the corresponding 
subsequence
$\left<v'_{h'}\ v'_{h'+1}\ \dots\ v'_m\right>$ of $p_i(t+1)$ of length $m-h'+1$ 
such that $n-h=m-h'$ (i.e., the two subsequences 
have the same length), $n-h+1\leq min(n,m)$, and $v_l=v'_{l-h+h'}$ for $l=h, 
\dots, n$. Considering again the example in Fig.~\ref{fig:path-example}, we 
have 
that $h=6$ and $h'=5$, because there are no more vertices before $v_6=v'_5=8$ 
along $p_i(t)$ and $p_i(t+1)$ that form a common subsequence ending at 
$v_7=v'_6=9$: therefore $c^\mathrm{tail}=\left<8\ 9\right>$. The 
common suffix has slightly different properties from the common 
prefix. 
Since $p_i(t)\neq p_i(t+1)$, it must always be
$c^\mathrm{tail}\neq p_i(t)$ and
$c^\mathrm{tail}\neq p_i(t+1)$. Moreover, it can also be 
$c^{\mathrm{tail}}=\left<\right>$, when at 
least one of $p_i(t)$ and $p_i(t+1)$ does not end at the intended destination 
$d$.

Based on these definitions, we can identify 
the 
parts of a traceroute path from $s$ to $d$ that change between consecutive time 
instants $t$ and $t+1$: let $\deltapre{i}{t}$ 
indicate the portion of path $p_i(t)$ that changes at time $t+1$, and 
$\deltapost{i}{t}$ indicate the portion of path $p_i(t+1)$ that has changed 
since time $t$. More formally, given two traceroute paths 
$p_i(t)$ and $p_i(t+1)$ such that $p_i(t)\neq p_i(t+1)$, $\deltapre{i}{t}$ is 
the subsequence of $p_i(t)$ such that 
$p_i(t)=c^\mathrm{head}\circ\deltapre{i}{t}\circ
c^\mathrm{tail}$, and $\deltapost{i}{t}$ is the subsequence of
$p_i(t+1)$ such that $p_i(t+1)=c^\mathrm{head}\circ 
\deltapost{i}{t}\circ c^\mathrm{tail}$.
Note that $\deltapre{i}{t}$ and $\deltapost{i}{t}$ always include 
the vertices, present in both $p_i(t)$ and $p_i(t+1)$, that delimit the changed subpath. 
Referring again to the example in Fig.~\ref{fig:path-example}, we have that 
$\deltapre{i}{t}=\left<2\ 3\ 4\ 5\ 8\right>$ and
$\deltapost{i}{t}=\left<2\ 6\ 7\ 8\right>$.


\subsection{Path Changes and Network Events}
One could argue that there 
could be several subsequences that are common to $p_i(t)$ and 
$p_i(t+1)$ 
besides the common prefix and the common suffix. In the example in 
Fig.~\ref{fig:nopolicy_twochanges} there is a common prefix 
$c^{\mathrm{head}}=\left<1\ 2\right>$, a common suffix
$c^{\mathrm{tail}}=\left<8\ 9\right>$, and an additional common 
subsequence 
$\left<5\ 6\right>$.
\begin{figure}
   \centering
   \includegraphics[scale=.85]{nopolicy}
   \caption{Scenario ruled out by Assumption~\ref{sa:nopolicy_contiguous}: a 
single event (failure of link $(7,8)$) causing changes at two 
non-contiguous portions of a traceroute path.}
   \label{fig:nopolicy_twochanges}
\end{figure}
In theory, our model comprises such additional 
subsequence within $\deltapre{i}{t}$ and $\deltapost{i}{t}$. However, in this 
example a single event, namely 
the failure of link $(7,8)$, causes changes of two non-contiguous portions of 
$p_i(t)$: $\left<2\ 3\ 4\ 5\right>$ is replaced by $\left<2\ 10\ 5\right>$ and
$\left<6\ 7\ 8\right>$ is replaced by $\left<6\ 11\ 8\right>$. While the 
change on the latter portion is clearly induced by the link 
failure, the 
change on the first portion is only possible if any vertices among $2$, $3$, 
$4$, $5$, and $10$ implement a routing policy that determines the selected path
based on the routing between $6$ and $8$, or if some  
policy change independent from the failure of link $(7,8)$ has 
occurred. Such routing policies could 
cause us to improperly consider traceroute path changes as related, and are
therefore ruled out by the following assumption.
\begin{assumption}[Continuous changed portion]
\label{sa:nopolicy_contiguous}
For any paths $p_i(t)$ and $p_i(t+1)$ such that $p_i(t)\neq p_i(t+1)$, 
it is always 
$V(\deltapre{i}{t})\cap V(\deltapost{i}{t})=\{v_1, v_n\}$, where
$\deltapre{i}{t}=\left<v_1\ \dots\ v_n\right>$ and
$\deltapost{i}{t}=\left<v_1\ \dots\ v_n\right>$.
\end{assumption}


In general, multiple traceroute paths can be influenced by a single event 
$E^\updown$. In order to better isolate the 
impact of each event, we make the following simplifying assumption.

\begin{assumption}[Non-interfering events]
\label{sa:simultaneous} 
Consider any two visible events $E_1^\updown$ and $E_2^\updown$ occurred at the 
same time $t$. For every $i\in S(E_1^\updown)$ and $j\in 
S(E_2^\updown)$, it must be $V(\deltapre{i}{t})\cap 
V(\deltapre{j}{t})=\emptyset$ and $V(\deltapost{i}{t})\cap 
V(\deltapost{j}{t})=\emptyset$.
\end{assumption}

This assumption imposes that events are ``independent enough'', thus enabling us 
to correctly handle and detect contemporary events. An immediate consequence of 
this assumption is that, 
for any two events $E_1^\updown$ and $E_2^\updown$, it must be 
$S(E_1^\updown)\cap S(E_2^\updown)=\emptyset$.

Real routing policies could be such that observed traceroute paths 
change because of an event that does not involve any edges along the paths (see 
for example~\cite{jcckak-pircipc-2013,fmzbm-liri-2004}). 
While this observation is quite relevant in a strict root-cause analysis setting, 
we rule them out here since root-cause analysis is not among our goals.
Further comments are in Section~\ref{sec:applicability}.

\begin{assumption}[Event on path]
\label{sa:nopolicy_eventonpath}
For any paths $p_i(t)$ and $p_i(t+1)$ such that $p_i(t)\neq p_i(t+1)$, 
there exists one event $E^\downarrow$ or $E^\uparrow$,
such that either $\deltapre{i}{t}$ contains at least a pair of consecutive 
vertices $(u,v)\in E^\downarrow$ or $\deltapost{i}{t}$ contains at least a 
pair of consecutive vertices $(u,v)\in E^\uparrow$.
\end{assumption}
A direct consequence of this assumption is that traceroute paths can only 
change if at least one event has occurred.

 \begin{figure}
    \centering
    \includegraphics[scale=.8]{no_hub}
    \caption{Path changes that, according to
    Assumptions~\ref{sa:simultaneous} and~\ref{sa:nopolicy_eventonpath}, cannot 
be caused by any combination of events. Paths at time $t$ are drawn thin and 
paths at time $t+1$ are drawn thick.}
    \label{fig:no_hub}
 \end{figure}


Fig.~\ref{fig:no_hub} shows a situation which 
is ruled out by Assumptions~\ref{sa:simultaneous} 
and~\ref{sa:nopolicy_eventonpath}.
This configuration cannot be produced by more than 
one event, by Assumption~\ref{sa:simultaneous}. On the other hand, by 
Assumptions~\ref{sa:nopolicy_eventonpath}, 
the only candidate for being a hub of a 
single event is vertex $5$. 
Edges $(3,5)$ and $(5,6)$ cannot be part of any event 
because they appear in traceroute paths both at time $t$ and at time $t+1$. The 
remaining 
edges cannot both belong to the same event, since $(4,5)$
is used a time $t+1$ and $(5,7)$ is used a time $t$.





==> 040-empathy.tex <==
\section{The Empathy Relation}\label{sec:empathy}
Now that we have defined $\deltapre{i}{t}$, and $\deltapost{i}{t}$, we can 
exploit them to introduce a relation, called \emph{empathy}, 
that determines when traceroute paths between different sd-pairs 
exhibit a similar behavior over time.

\subsection{Pre-Empathy and Post-Empathy}
Let $p_1(t)$ be a traceroute path measured by $s_1$ towards $d_1$ at time $t$ 
and $p_2(t)$ be a traceroute path measured by $s_2$ towards $d_2$ at the same 
time. Also let $p_1(t+1)$ and $p_2(t+1)$ be the traceroute paths measured at 
time $t+1$ between the same sd-pairs.
We say that \emph{$(s_1,d_1)$ and $(s_2,d_2)$ are pre-empathic at time 
$t$}, indicated with $(s_1,d_1)\preemp{t}(s_2,d_2)$, if:
\begin{enumerate}
\item the two traceroute paths $p_1$ and $p_2$ change between $t$ and $t+1$, 
namely $p_1(t)\neq p_1(t+1)$ and $p_2(t)\neq p_2(t+1)$;
\item the portions of $p_1(t)$ and $p_2(t)$ that change at $t+1$ overlap, 
namely $V(\deltapre{1}{t})\cap V(\deltapre{2}{t})\neq\emptyset$.

\end{enumerate}

Similarly, we say that \emph{$(s_1,d_1)$ and $(s_2,d_2)$ are 
post-empathic at time $t$}, indicated with $(s_1,d_1)\postemp{t} 
(s_2,d_2)$, if $p_1(t)\neq p_1(t+1)$ and 
$V(\deltapost{1}{t})\cap V(\deltapost{2}{t})\neq\emptyset$.

Relations $\preemp{}$ and \ $\postemp{}$ are, trivially, commutative and reflexive.

Intuitively, distinguishing the pre-empathy from the post-empathy allows us to 
get a more accurate picture of how the traceroute paths between two 
sd-pairs change between $t$ and $t+1$: if two sd-pairs are pre-empathic, 
their traceroute paths stop traversing a portion 
that they shared before the event occurred; if two sd-pairs are 
post-empathic, their traceroute paths start traversing a common portion 
that they did not use before the event occurred.
An example showing how to determine empathies is shown in 
Fig.~\ref{fig:empathy_examples}. There are two traceroute paths 
$p_1$, from $s_1$ to $d_1$, and $p_2$, from $s_2$ to $d_2$, and the event that 
causes these paths to change between $t$ and $t+1$ is the failure of link 
$(5,6)$. In this example we have 
$\deltapre{1}{t}=\left<5\ 6\right>$,
$\deltapost{1}{t}=\left<5\ 9\ 6\right>$,
$\deltapre{2}{t}=\left<4\ 5\ 6\ 8\right>$, and
$\deltapost{2}{t}=\left<4\ 10\ 8\right>$. It is now easy to observe that
$(s_1,d_1)\preemp{t}(s_2,d_2)$, because 
$V(\deltapre{1}{t})\cap V(\deltapre{2}{t})=\{5,6\}$. On the other hand, despite 
the fact 
that 
$p_1(t+1)$ and $p_2(t+1)$ have common subpaths, $(s_1,d_1)$ and 
$(s_2,d_2)$ are not post-empathic, because 
$V(\deltapost{1}{t})\cap V(\deltapost{2}{t})=\emptyset$.
This is an indication of the fact that $p_1$ and $p_2$ behave similarly before 
the event happens and change to two 
independent routes after the event has happened.

\begin{figure}
   \centering
   \includegraphics[scale=.8]{empathy-examples}
   \caption{An example showing empathy relations. In this 
scenario link $(5,6)$ fails, and we have $(s_1,d_1)\preemp{t}(s_2,d_2)$ but 
$(s_1,d_1)\not\postemp{t}(s_2,d_2)$.}
   \label{fig:empathy_examples}
\end{figure}


Assumption~\ref{sa:nopolicy_contiguous} rules out traceroute paths having 
unchanged portions that do not belong to the common prefix or suffix. Therefore, 
it prevents us from improperly considering an overlap of such portions as an 
evidence of empathy between the corresponding sd-pairs.
Moreover, under Assumptions~\ref{sa:simultaneous} 
and~\ref{sa:nopolicy_eventonpath} the following property holds.


\begin{property}\label{pro:event_clique}
   If a visible event $E^\downarrow$ (respectively, $E^\uparrow$) occurs at 
time $t$, then for every $i,j\in S(E^\downarrow)$ 
(respectively, $i,j\in S(E^\uparrow)$), we have that $i\preemp{t}j$ 
(respectively, 
   $i\postemp{t}j$).
\end{property}
\begin{IEEEproof}
The property holds because, by definition, the hubs of $E^\downarrow$ 
appear in $\deltapre{i}{t}$ for any $i\in S(E^\downarrow)$, and
the hubs of $E^\uparrow$ appear in $\deltapost{j}{t}$ for any $j\in 
S(E^\uparrow)$.
\end{IEEEproof}


\subsection{Empathy Graphs}
Being a natural representation for a relation, we conveniently model 
empathies between sd-pairs using a graph. We call 
$\empgraphpre{t}=(\empgraphvpre{t},\empgraphepre{t})$  
the \emph{pre-empathy graph at time $t$}, where each vertex $v=(s,d)\in 
\empgraphvpre{t}$ is a sd-pair and there is an edge between 
$(s_1,d_1)\in \empgraphvpre{t}$ and $(s_2,d_2)\in 
\empgraphvpre{t}$ if and only if $(s_1,d_1)\preemp{t}(s_2,d_2)$. Likewise, we 
define  the 
\emph{post-empathy graph at time $t$}, 
$\empgraphpost{t}=(\empgraphvpost{t},\empgraphepost{t})$, relying on~~$\postemp{t}$.

We exploit the empathy graph in order to single out network events, but a 
few additional properties are needed.
\begin{property}\label{pro:vertex_in_scope}
For any vertex $v\in \empgraphvpre{t}$ (respectively, $\empgraphvpost{t}$) 
there is an event $E^\updown$ at 
time $t$ such that $v\in S(E^\updown)$.
\end{property}
\begin{IEEEproof}
By definition of empathy, the existence of a vertex $i$ in 
$\empgraphvpre{t}$ implies that $p_i(t)\neq p_i(t+1)$. Therefore, by 
Assumption~\ref{sa:nopolicy_eventonpath}, there is an event $E^\updown$ 
which caused path $p_i$ to change, and vertex $i$ is obviously in the scope of 
$E^\updown$.
\end{IEEEproof}

\begin{property}\label{pro:events_noempathy}
Consider two visible events $E_1^\updown$ and $E_2^\updown$ 
occurred at time $t$. For any two vertices $u\in S(E_1^\updown)$ 
and $v\in S(E_2^\updown)$ it must be $(u,v)\notin\empgraphepre{t}$ and 
$(u,v)\notin\empgraphepost{t}$.
\end{property}
\begin{IEEEproof}
The statement follows from Assumption~\ref{sa:simultaneous}.
\end{IEEEproof}



\subsection{Cliques in the Empathy Graphs}
Property~\ref{pro:event_clique} suggests an interesting observation: if a visible 
event $E^\updown$ occurs at time $t$ in the network,
then a clique is formed in an empathy graph at time $t$ (we recall that a 
clique is a structure in a 
graph such that there is an edge between any two distinct vertices).

In order to turn this observation into a statement, we introduce the 
following concept:
given a set $C\subseteq\empgraphvpre{t}$ of 
vertices of $\empgraphpre{t}$,
we call \emph{pivot set} 
of $C$ a set $\pipre{C}\subset V$ such that, for every 
$v\in\pipre{C}$, it is
$v\in\deltapre{i}{t}$ for all $i\in C$. By construction, the pivot set of a 
set $C$ of vertices in $\empgraphvpre{t}$ can only be non-empty if 
vertices of $C$ form a 
clique in the pre-empathy graph, namely $(u,v)\in\empgraphepre{t}$ for any 
$u,v\in C$. We also naturally define a pivot set $\pipost{C'}$ for every 
set $C'$ of vertices in the post-empathy graph $\empgraphpost{t}$. Intuitively, 
given a group of traceroute paths that behave similarly to each other, the pivot 
is the set of vertices that appear in the changed portions of all these paths.
We now state the most important properties of the empathy graph, which we use in 
Section~\ref{sec:methodology} to devise an algorithm that searches for events 
based on the observed traceroute paths.

\begin{theorem}\label{the:event>clique}
For every visible event $E^\downarrow$ occurred at time 
$t$ the following conditions hold:
\begin{inparaenum}[i)]
\item there exists one clique in $\empgraphpre{t}$, namely a set 
$C\subseteq\empgraphvpre{t}$ of vertices such that, for every $u_1,u_2\in C$ 
there 
is an edge $(u_1,u_2)\in\empgraphepre{t}$;
\item $C=S(E^\downarrow)$;
\item $\pipre{C}\neq\emptyset$;
\item $C$ forms an isolated connected component in $\empgraphpre{t}$, namely 
for any two vertices $v\in C$ and $w\in\empgraphvpre{t}\backslash C$ it is 
$(v,w)\notin\empgraphepre{t}$.
\end{inparaenum}
The statement also applies to an event $E^\uparrow$, by replacing 
$\empgraphpre{t}=(\empgraphvpre{t},\empgraphepre{t})$ with
$\empgraphpost{t}=(\empgraphvpost{t},\empgraphepost{t})$.
\end{theorem}
\begin{IEEEproof}
Suppose there is a visible event $E^\downarrow$ at time $t$. By definition of 
visible event and by Property~\ref{pro:event_clique}, there must be a set $C$ 
of vertices in $\empgraphvpre{t}$ that form a clique. As stated in the proof of 
Property~\ref{pro:event_clique}, the hub of $E^\downarrow$ must appear in 
$\deltapre{u}{t}$ for every $u\in C$, which also implies that 
$\pipre{C}\neq\emptyset$. By construction, every vertex in 
$S(E^\downarrow)$ is part of the clique, namely $C=S(E^\downarrow)$, and 
for every other vertex $w\in\empgraphvpre{t}\backslash C$, for which by 
Property~\ref{pro:vertex_in_scope} there exists an event $\bar E^\updown$ at 
time $t$ such that $w\in S(\bar E^\updown)$, it must be $\bar E^\updown\neq 
E^\updown$. By Property~\ref{pro:events_noempathy}, this also excludes the 
existence of any edges $(v,w)\in\empgraphepre{t}$, with $v\in C$.
The same arguments apply for an event $E^\uparrow$.
\end{IEEEproof}



The following theorems establish a relationship between the structures of 
$\empgraphpre{t}$ and $\empgraphpost{t}$, which we also use in the 
algorithm in Section~\ref{sec:methodology}.
\begin{theorem}\label{the:cliquepre>ccpost}
If there exists a visible event $E^\downarrow$ (respectively, $E^\uparrow$) at 
time 
$t$, then every set $C$ of vertices in $\empgraphpost{t}$ (respectively, 
$\empgraphpre{t}$) that form a connected component with at least one vertex in 
$S(E^\downarrow)$ (respectively, $E^\uparrow$) is such that $C\subseteq 
S(E^\downarrow)$ (respectively, $C\subseteq S(E^\uparrow)$).
\end{theorem}
\begin{IEEEproof}
Assume that there is a visible event $E^\downarrow$ at time $t$ and suppose, by 
contradiction, that one of the connected components in $\empgraphpost{t}$ is 
formed by a set $C$ of vertices such that one vertex $v\in C$ is in 
$S(E^\downarrow)$ and another vertex $w\in C$ is not in $S(E^\downarrow)$. By 
Property~\ref{pro:vertex_in_scope}, there must be another event $\bar 
E^\updown\neq E^\updown$ such that $w\in S(\bar E^\updown)$, leading to an 
absurd because, by Property~\ref{pro:events_noempathy}, edge 
$(v,w)\in\empgraphepost{t}$ should not exist.
Similar arguments can be applied for an event $E^\uparrow$.
\end{IEEEproof}

From Theorems~\ref{the:event>clique} and~\ref{the:cliquepre>ccpost}
it is possible to deduce that the structure of 
$\empgraphpre{t}$ and $\empgraphpost{t}$ in the presence of network events is 
the following:
%the one in Fig.~\ref{fig:empgraph_prepost}:
for each event $E^\downarrow$ there 
is an isolated clique in $\empgraphpre{t}$ that spans all sd-pairs in 
$S(E^\downarrow)$, and one or more connected components in $\empgraphpost{t}$ 
that are formed by sd-pairs in $S(E^\downarrow)$. Our algorithm 
in Section~\ref{sec:methodology} is based on recognizing such patterns in 
$\empgraphpre{t}$ and $\empgraphpost{t}$.

The following property is another direct consequence of 
Theorems~\ref{the:event>clique} and~\ref{the:cliquepre>ccpost}.
\begin{property}
Given any two events $E_1^\updown$ and $E_2^\updown$ occurred at time $t$, it 
is always $\pipre{S(E_1^\updown)}\cap\pipre{S(E_2^\updown)}=\emptyset$ and 
$\pipost{S(E_1^\updown)}\cap\pipost{S(E_2^\updown)}=\emptyset$.
\end{property}
\begin{IEEEproof}
The statement immediately follows by considering that, by 
Theorem~\ref{the:event>clique}, cliques in $\empgraphpre{t}$ or in 
$\empgraphpost{t}$ corresponding to distinct events are isolated from each 
other and, by Theorem~\ref{the:cliquepre>ccpost}, the same isolation applies to
any other connected components in $\empgraphpre{t}$ or in $\empgraphpost{t}$.
\end{IEEEproof}


The following two theorems state that network events can be pointed out by 
searching for cliques in empathy graphs.


\begin{theorem}\label{the:event<clique}
If a set $C\in\empgraphvpre{t}$ of at least 2 sd-pairs forms a 
maximal clique in 
$\empgraphpre{t}$ and it is $\pipost{C}=\emptyset$, then 
$\pipre{C}\neq\emptyset$ and there is a unique 
visible event $E^\downarrow$ at time $t$ whose hubs are in $\pipre{C}$.
The theorem can be restated by swapping
$\empgraphpre{t}$ with $\empgraphpost{t}$, $\empgraphvpre{t}$ with 
$\empgraphvpost{t}$, $\pipre{C}$ with 
$\pipost{C}$, and $E^\downarrow$ with $E^\uparrow$.
\end{theorem}
\begin{IEEEproof}
Consider a clique $C\in\empgraphvpre{t}$ consisting of at least 2 sd-pairs and 
such that $\pipost{C}=\emptyset$.
By Assumption~\ref{sa:nopolicy_eventonpath}, at least one event $E^\updown$ 
whose scope involves sd-pairs in $C$ must have occurred at time $t$, and this 
event is obviously visible. In addition, because sd-pairs in $C$ form a clique 
in $\empgraphpre{t}$, there can be no more than one event $E^\updown$ whose 
scope involves sd-pairs in $C$, otherwise Assumption~\ref{sa:simultaneous} is 
violated. This, together with the fact that the clique is maximal, implies 
that $S(E^\updown)=C$. Since $\pipost{C}=\emptyset$, 
there is no way of constructing a single up event $E^\uparrow$ such that 
$S(E^\uparrow)=C$, therefore there must exist a unique down event $E^\downarrow$ 
at time $t$ such that $S(E^\downarrow)=C$. Finally, since 
$E^\downarrow$ is unique, $\pipre{C}$ cannot be empty and must contain the 
hubs for $E^\downarrow$.
\end{IEEEproof}


\begin{theorem}\label{the:unknown<clique}
If a set $C$ of at least 2 sd-pairs forms a maximal clique in 
$\empgraphpre{t}$ such that $\pipre{C}\neq\emptyset$ and a clique in
$\empgraphpost{t}$ such that $\pipost{C}\neq\emptyset$, then there exists a 
unique visible event $E^\updown$ at time $t$ whose hubs are in 
$\pipre{C}\cup\pipost{C}$.
\end{theorem}
\begin{IEEEproof}
By exploiting Assumptions~\ref{sa:simultaneous} 
and~\ref{sa:nopolicy_eventonpath} and applying arguments similar 
to those used in the 
proof of Theorem~\ref{the:event<clique}, we can deduce that there exists exactly 
one event in $E^\updown$ at time $t$ and, since $E^\updown$ is unique, the hubs 
of $E^\updown$ must be contained in $\pipre{C}\cup\pipost{C}$.
Differently from Theorem~\ref{the:event<clique}, it is not possible to 
disambiguate the type of event, because $\pipre{C}\neq\emptyset$ and 
$\pipost{C}\neq\emptyset$.
\end{IEEEproof}


We now exploit Fig.~\ref{fig:empathy_examples} to make an
example of application of Theorem~\ref{the:event<clique}.

In this figure we only have a clique 
$C=\{(s_1,d_1),(s_2,d_2)\}$ in $\empgraphpre{t}$ and no cliques in 
$\empgraphpost{C}$, therefore it is $\pipost{C}=\emptyset$. Indeed, in this 
example we have  $\pipre{C}=\{5,6\}$, and it can be easily 
checked that both $5$ and $6$ are hub vertices for the event 
$E^\downarrow=\{(5,6)\}$ which has actually occurred at time $t$.



In order to find traceroute paths that behave similarly over time, we need to 
search for events that may have influenced these paths. The above theorems 
suggest that hubs for these events can be searched in the pivot set of 
maximal cliques in $\empgraphpre{t}$ or $\empgraphpost{t}$. Vice versa, 
IP addresses occurring in $\deltapre{i}{t}$ or $\deltapost{i}{t}$ of many sd-pairs $i$
provide strong hints about the existence of maximal cliques. These properties are 
at the basis of the methodology described in Section~\ref{sec:methodology}.

==> 070-applicability.tex <==
\section{Applicability Considerations}\label{sec:applicability}

In this section we discuss some hypothesis we rely on and their impact on the 
results of our approach.

\subsection{Time-Related Assumptions}

There are two more assumptions that have been implicitly made regarding time:
\begin{inparaenum}
\item the internal clock of the probes is properly set, and
\item an event is instantly propagated to the entire network.
\end{inparaenum}
The internal clock of the probes is usually kept synchronized by NTP, whose 
precision is quite high with respect to the needs of our methodology, even in the 
case
of asymmetric bandwidth lines like ADSL. So, we think this is not a relevant issue.

Regarding the delay in the dissemination of routing messages, it is well known 
that 
certain routing events  take some time to propagate (e.g. BGP advertisements 
might be delayed by the MRAI timer, by 30 seconds according to the standard). 
On the other hand, link state routing 
protocols, like OSPF, are much faster to converge.
So, when BGP is involved, at a given time some routers may
see (and propagate) a stale version of the routing.  
In this case, it might happen that not all transitions overlap on a common 
interval (see
Section~\ref{sec:methodology}), with the effect of having multiple inferred 
events usually with many sd-pairs in common.

\iffalse
Assumption~\ref{sa:simultaneous} also involves timing. It mandates that two 
distinct events should neither overlap in time nor in the changes they 
induce on traceroute paths.

It is clear that in 
real world data this assumption may not hold. 
Two interfering events may lead to several effects. 
First, it is no longer true that distinct down (up) events lead to distinct 
connected components in $\empgraphpre{t}$ ($\empgraphpost{t}$), as stated in Theorem~\ref{the:event>clique}, but, since 
our methodology starts from elements of the pivot set, it is likely to still infer 
the right events. However, IP addresses involved in more than one event induce inference of 
fictitious events having as inferred scope the interfering sd-pairs.
Second, it is no longer true that for each down (up) event with scope $S$ there are in 
$\empgraphpost{t}$ ($\empgraphpre{t}$) several connected components contained in $S$ 
(Theorem~\ref{the:cliquepre>ccpost}).
E.g., two down events can have sd-pairs with interfering $\deltapost{}{t}$. This results in 
fictitious up events for the interfering sd-pairs. 

Another relevant effect of interference is the skewing of the timings of the 
inferred events. It might happen that a large number of sd-pairs agree on 
an event $E^\updown$ with interval $(t_1, t_2)$ and just a single distinct 
sd-pair 
interferes, because of another event, with interval $(t_2-\epsilon, t_3)$. In 
this case our methodology reports only one event with interval 
$(t_2-\epsilon,t_2)$ which might be quite distant from the instant in which the 
real event happened. This kind of behavior can be observed in the experimental
results in Section~\ref{sec:experiments}.
\fi

\subsection{Handling Load Balancers}\label{sec:loadbalancers}

Load balancers cannot be ignored in our analysis, since they are the cause 
of many routing changes which are reported as events by our algorithm while they are 
usually not interesting. Our approach for handling load balancers is to suppose they are 
known and to pre-process the traceroutes to substitute each IP address belonging 
to a load balancer with one fixed representative address.

We claim that such assumption is not dramatic.
First, an ISP willing to apply our methodology already knows the load balancers in its network.
Second, \emph{Paris Traceroute} \cite{augustin2007paris} is a well-known variation of the traceroute measurement that is able to find load balancers by
exhaustively exploring routing paths in a network. This kind of measurement 
can be potentially implemented in the same probes that perform traceroutes to 
gather this information.

The probes used in the experiment considered in Section~\ref{sec:experiments} do not 
support Paris Traceroute, so we applied a very rough heuristic to detect load balancers 
using data produced by standard traceroutes, which performed well enough for our 
evaluation purposes.
We analyzed traceroutes in a time-ordered manner. For each destination
we learned the routing of all nodes that appear in each traceroute and their evolution over time.
We computed some simple statistics on route changes for each node. Neighbors that 
are not ``stable'' enough (in our case when more than 20\% of the samples are 
changes) are considered to belong to a load balancer.
